Align on the Fly: Adapting Chatbot Behavior to Established Norms

In this paper, we aim to align large language models with the ever-changing, complex, and diverse human values (e.g., social norms) across time and locations. This presents a challenge to existing alignment techniques, such as supervised fine-tuning, which internalize values within model parameters. To overcome this, we propose an On-the-fly Preference Optimization (OPO) method, which is a real-time alignment that works in a streaming way. It employs an external memory to store established rules for alignment, which can constrain LLMs' behaviors without further training, allowing for convenient updates and customization of human values. We also introduce a scalable evaluation to assess the proposed method more effectively. Experimental results on both human-annotated and auto-generated questions from legal and moral domains indicate the effectiveness of the proposed OPO method. Our code and data are released at https://github.com/GAIR-NLP/OPO.

==> figures_tex_files/introduction_case.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=2\columnwidth]{figures/introduction_case_morality.pdf}
% \includegraphics[width=2\columnwidth]{figures/introduction_case_politics.pdf}
% \vspace{-2em}
\caption{A question example and the retrieved morality rules. Note that answer of retrieval-argumented GPT-4 is correct while the answer of original GPT-4 is wrong. \xu{This case might be not good enough. I would select another case.}}
% \vspace{-1.5em}
\label{fig:intro_case}
\end{figure*}

==> figures_tex_files/question-generation-framework.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.7\columnwidth]{figures/question-generation-framework.pdf}
% \includegraphics[width=2\columnwidth]{figures/introduction_case_politics.pdf}
% \vspace{-2em}
\caption{The scalable question-generation framework.}
% \vspace{-1.5em}
\label{fig:question-generation-framework}
\end{figure*}

==> figures_tex_files/translated_question_generation_prompt.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=2\columnwidth]{figures/translated_question_generation_prompt.pdf}
% \includegraphics[width=2\columnwidth]{figures/introduction_case_politics.pdf}
% \vspace{-2em}
\caption{The specially designed prompt for generating questions, explanations, and answers.}
% \vspace{-1.5em}
\label{fig:translated_question_generation_prompt}
\end{figure*}

==> sections/dataset.tex <==

% \section{Rule data collection}
% \subsection{Legal Rules}
% We collect legal data from the National Database of Laws and Regulations (NDLR) \footnote{\url{https://flk.npc.gov.cn}} and National Database of Government Regulations (NDGR) \footnote{\url{https://www.gov.cn/zhengce/xxgk/gjgzk/ssgz.htm}}, which mostly cover all laws and regulations currently in force in China.
% %\footnote{The legislative system in China is provided with a detailed introduction in \url{https://www.gov.cn/guoqing/2017-11/08/content_5238056.htm}}. 
% The former contains the Constitution, Laws, Administrative Regulations, Supervisory Regulations, Judicial Interpretation, and Local Regulations while the latter consists of the Departmental Rules of the State Council and Local Government Regulations. 

% \subsection{Moral Rules}
% Unlike legal rules, which are explicitly defined and established by government legislatures, moral rules are typically rooted in social norms and cultural values. These moral guidelines are often composed of implicit soft constraints.

% Inspired by that students learn about basic moral theories through the subject of Morality and Law, we utilize middle school textbooks on this subject, sourced from the Smart Education Platform~\footnote{\url{https://basic.smartedu.cn}}, to extract data on morality. Specifically, we filter out the legal content from these textbooks, focusing solely on extracting moral guidelines from the remaining material.
% The moral rules collected from textbooks are mainly about personal morality and social norms. Due to the reason professional ethics is an important part of morality~\cite{turner2013professional}, we collect professional ethics codes from 57 different companies and industries online.





% \subsection{Rule processing}
% The data collected from NDLR is available in several formats, including PDF and Microsoft Word files while the data from NDGR mainly comes in the format of web pages.
% We convert the PDF documents into Word files, extract the laws from these files, and store them according to the sequence of the law numbers. For web pages, we directly extract laws from the raw texts.
% The data sourced from NDLR is accessible in multiple formats, mainly PDF and Microsoft Word documents, while the data from NDGR mostly exists in web page format. We convert the PDFs into Word documents, extract legal statutes, and systematically organize them by their respective law numbers. For web pages, we directly obtain the laws from their raw text content.



% % The sequence number is explicitly contacted with the law text as shown in Figure \ref{fig:data_case}.

% The textbooks are cluttered with extraneous information, requiring careful data-cleansing efforts. Initially, we remove chapters related to law, as legal materials are covered by the NDLR and NDGR databases. This allows us to concentrate on collecting moral rules from the textbooks. Furthermore, we refine the material by retaining only the principal texts and discarding supplementary contents such as figures and discussions. Lastly, we treat each paragraph in the main texts as an individual moral rule, categorizing and numbering them by chapter.
% Similarly, we process and number the professional moral rules from the collected professional ethics codes. The examples of the collected law and moral rules are shown in Figure \ref{fig:rule_case}, and the analysis of the collected rules can be found in Table \ref{tab:retrieval_data_details}.

\subsection{Evaluation Module}
The pre-training and SFT of LLMs often involve extensive text data that is typically non-public, raising concerns about benchmark leakage ~\cite{Benchmark_Cheater_HanJiawei_arxiv2023}, 
which refers to the inadvertent use of data from evaluation sets in training, potentially disturbing the fairness in comparing LLMs' performance.
Meanwhile, a small portion of Chinese laws (e.g., Constitution and Criminal Law) are covered in the questions collected from law exams while many laws are not included, particularly the local laws. It's difficult to collect human-annotated questions related to these laws. Besides, there are no evaluation benchmarks considering evaluating the professional ethics of LLMs, but a critical aspect of morality. Therefore, to alleviate the benchmark leakage problem and enhance the comprehensiveness of evaluation, we propose an evaluation module to automatically generate new legal questions and professional moral questions by utilizing the powerful LLM (i.e., GPT-4). Clearly, we first collect a set of questions as the seed questions, each of which consists of a question stem, four options, a detailed analysis, the rules applied in solving the question, and the correct answer. These seed questions serve as practical demonstrations for in-context learning \cite{ICL-NIPS2020}. An example of seed questions is shown in Figure \ref{fig:seed_question}. 
Additionally, we leverage our collected text corpus to provide relevant contexts for the generation of new questions.

Specifically, a rule is randomly selected from the text corpus and top-$l$ similar rules are obtained via k-Nearest-Neighbor (kNN) retrieval to enrich the content. The randomly selected rule is then concatenated with the $l$ similar rules to form the final context for question generation. To improve the diversity of the generated questions, we randomly select a question from the seed question set. Then we meticulously design a question generation prompt that includes 13 detailed requirements. GPT-4 is employed to generate a question based on the provided seed question and combined context. Additionally, Chain-of-thought (COT) reasoning \cite{COT_Kojima_nips2022,COT_wei_nips2022} is employed to improve the quality of the generated questions. The generated question contains the question stem, options, analysis, and correct answer. We demonstrate the question generation prompt in Figure \ref{fig:question_generation_prompt} and the generated question example in Figure \ref{fig:generated_question_example}.
To ensure the high quality of the generated questions, we use another GPT-4 to evaluate each component of the question. This evaluation process employs the same rules that are used to generate the question. We collect the question only if it satisfies all criteria in these four areas; otherwise, we will discard it. The quality evaluation prompt is provided in Figure \ref{fig:question_quality_evaluation_prompt}. Note that many efforts are made to design both the question generation prompt and quality evaluation prompt. We test a small portion of the data, manually check the results, and iteratively revise the prompts based on the analysis of bad cases until we achieve satisfactory results.


% \input{figures_tex_files/question-generation-framework}

% \subsection{Auto-generated data} 
% The pre-training and SFT of LLMs often involve extensive text data that is typically non-public, raising concerns about benchmark leakage ~\cite{Benchmark_Cheater_HanJiawei_arxiv2023}, 
% which refers to the inadvertent use of data from evaluation sets in training, potentially disturbing the fairness in comparing LLMs' performance.
% Meanwhile, a small portion of Chinese laws (e.g., Constitution and Criminal Law) are covered in the questions collected from law exams while many laws are not included, particularly the local laws. It's difficult to collect human-annotated questions related to these laws. Besides, there are no evaluation benchmarks considering evaluating the professional ethics of LLMs, but a critical aspect of morality. Therefore, to alleviate the benchmark leakage problem and enhance the comprehensiveness of evaluation, we propose an evaluation module to automatically generate new legal and professional moral questions by utilizing the powerful LLM (i.e., GPT-4). Clearly, we first collect a set of questions as the seed questions, each of which consists of a question stem, four options, a detailed analysis, the rules applied in solving the question, and the correct answer. These seed questions serve as practical demonstrations for in-context learning \cite{ICL-NIPS2020}. An example of seed questions is shown in Figure \ref{fig:seed_question}. 
% Additionally, we leverage our collected text corpus to provide relevant contexts for the generation of new questions.

% Specifically, a rule is randomly selected from the text corpus and top-$l$ similar rules are obtained via k-Nearest-Neighbor (kNN) retrieval to enrich the content. The randomly selected rule is then concatenated with the $l$ similar rules to form the final context for question generation. To improve the diversity of the generated questions, we randomly select a question from the seed question set. Then we meticulously design a question generation prompt that includes 13 detailed requirements. GPT-4 is employed to generate a question based on the provided seed question and combined context. Additionally, Chain-of-thought (COT) reasoning \cite{COT_Kojima_nips2022,COT_wei_nips2022} is employed to improve the quality of the generated questions. The generated question contains the question stem, options, analysis, and correct answer. We demonstrate the question generation prompt in Figure \ref{fig:question_generation_prompt} and the generated question example in Figure \ref{fig:generated_question_example}.
% To ensure the high quality of the generated questions, we use another GPT-4 to evaluate each component of the question. This evaluation process employs the same rules that are used to generate the question. We collect the question only if it satisfies all criteria in these four areas; otherwise, we will discard it. The quality evaluation prompt is provided in Figure \ref{fig:question_quality_evaluation_prompt}. Note that many efforts are made to design both question generation prompt and quality evaluation prompt. We test a small portion of the data, manually check the results, and iteratively revise the prompts based on the analysis of bad cases until we achieve satisfactory results.

\input{figures_tex_files/question_generation_prompt}
\input{figures_tex_files/question_quality_evaluation_prompt}
\input{figures_tex_files/generated_question_example}

==> tables/main_results_law_original_questions.tex <==
\begin{table*}[t]
\centering
\resizebox{1.8\columnwidth}{!}{
    \begin{tabular}[b]{l m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering}}
    \toprule[1pt]
    \multirow{2}*{\textbf{Models}} &  \multicolumn{2}{c}{\textbf{H-Law}} & \multicolumn{3}{c}{\textbf{A-Law}} \\
    \cmidrule(r){2-3} \cmidrule(r){4-6}
        &Base  & Retrieval   &Base & Retrieval & Oracle  \\
    \midrule[0.7pt]
    \textit{\textbf{Closed-source models}} \\
    \midrule[0.7pt]
    % Claude-v1.3 &       &       &       &       &  \\
    % claude-v2 &       &       &       &       &  \\
    ChatGPT & 41.62 & 48.07 & 75.11 & 83.12 & 86.58 \\
    GPT-4 & 57.21 & 62.25 & 80.74 & 92.42 & 96.32 \\
    \midrule[0.7pt]
    \textit{\textbf{Open-source models}} \\
    \midrule[0.7pt]
    ChatGLM2-6B & 47.71 & 45.96 & 76.19 & 82.25 & 82.68 \\
    ChatGLM3-6B & 49.53 & 51.58 & 76.41 & 80.74 & 83.12 \\
    InternLM-Chat-6B & 46.13 & 48.3  & 72.29 & 81.17 & 82.47 \\
    Llama2-Chat-7B & 31.48 & 28.37 & 58.87 & 61.26 & 61.9 \\
    Qwen-Chat-7B & 52.46 & 53.63 & 78.57 & 84.2  & 88.31 \\
    XVERSE-Chat-7B & 47.3  & 52.99 & 75.76 & 86.15 & 86.8 \\
    DISC-LawLLM-13B & 50.41 & 52.58 & 76.84 & 82.25 & 84.85 \\
    Llama2-Chat-13B & 30.3  & 35.99 & 65.37 & 75.11 & 77.27 \\
    XVERSE-Chat-13B & 48.01 & 54.57 & 74.89 & 85.28 & 87.88 \\
    Qwen-Chat-14B & 62.43 & 66.82 & 82.47 & 90.04 & 90.04 \\
    InternLM-Chat-20B & 47.6  & 51.93 & 73.38 & 84.2  & 87.01 \\
    LLaMA2-Chat-70B & 35.11 & 39.1  & 65.37 & 79    & 85.28 \\
    XuanYuan-70B & 65.42 & 70.22 & 81.6  & 91.34 & 92.64 \\
    %LaWGPT-7B & & & & & & \\
    %Lawyer-Llama-13B & & & & & & \\
    %ChatLaw-33B & & & & & & \\
    
    \bottomrule[1pt]	
    \end{tabular}
}
% \vspace{-1em}
\caption{The accuracy of evaluated LLMs on H-Law and A-law without human filtering. ``Base'' column indicates the original performance of each LLM. ``Retrieval'' column represented the performance of each LLM argumented by the retrieval. Here we show the results with a maximum retrieval context length of up to 1000 for fair comparisons. ``Oracle'' column stands for the results of using rules, utilized to generate the questions, to argument the LLM.}
\label{tab:law_results}
\end{table*}

==> tables/main_results_morality_questions.tex <==
\begin{table*}[t]
\centering
\resizebox{1.8\columnwidth}{!}{
    \begin{tabular}[b]{l m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering} m{0.12\textwidth}<{\centering}}
    \toprule[1pt]
    \multirow{2}*{\textbf{Models}} &  \multicolumn{2}{c}{\textbf{H-Law}} & \multicolumn{3}{c}{\textbf{A-Law}} \\
    \cmidrule(r){2-3} \cmidrule(r){4-6}
        &Base  & Retrieval   &Base & Retrieval & Oracle  \\
    \midrule[0.7pt]
    \textit{\textbf{Closed-source models}} \\
    \midrule[0.7pt]
    % Claude-v1.3 &       &       &       &       &  \\
    % claude-v2 &       &       &       &       &  \\
    ChatGPT & 64.37 & 63.43 & 52.3  & 64.2  & 90.07 & 92.65 & 93.38 \\
    GPT-4 & 84.62 & 86.37 & 56.9  & 69.9  & 95.96 & 97.43 & 99.26 \\
    \midrule[0.7pt]
    \textit{\textbf{Open-source models}} \\
    \midrule[0.7pt]
    ChatGLM2-6B & 83.67 & 83.54 & 46.3  & 53.25 & 85.66 & 90.81 & 90.81 \\
    ChatGLM3-6B & 83.81 & 82.59 & 39.3  & 44.65 & 88.6  & 91.54 & 91.91 \\
    InternLM-Chat-6B & 87.85 & 88.26 & 47.8  & 56.15 & 88.6  & 91.54 & 94.49 \\
    Llama2-Chat-7B & 35.36 & 34.95 & 29.45 & 45.45 & 70.59 & 73.53 & 79.04 \\
    Qwen-Chat-7B & 90.15 & 90.96 & 46.5  & 58.8  & 89.71 & 93.38 & 95.96 \\
    XVERSE-Chat-7B & 82.46 & 84.62 & 47.4  & 54.55 & 91.18 & 94.85 & 94.85 \\
    DISC-LawLLM-13B & 70.72 & 68.96 & 51.65 & 60.65 & 88.24 & 91.18 & 90.81 \\
    Llama2-Chat-13B & 42.78 & 44.8  & 35.75 & 56.8  & 75.74 & 82.35 & 82.35 \\
    XVERSE-Chat-13B & 79.49 & 81.51 & 49.3  & 61.5  & 87.87 & 91.54 & 93.38 \\
    Qwen-Chat-14B & 93.79 & 94.47 & 49.15 & 64.6  & 94.85 & 97.79 & 98.16 \\
    InternLM-Chat-20B & 87.99 & 86.91 & 46.85 & 62.4  & 90.07 & 93.01 & 94.49 \\
    LLaMA2-Chat-70B & 48.72 & 53.58 & 45.15 & 62.25 & 88.97 & 91.18 & 94.12 \\
    XuanYuan-70B & 93.52 & 94.06 & 54.9  & 64.1  & 96.69 & 98.53 & 98.9 \\
    %LaWGPT-7B & & & & & & \\
    %Lawyer-Llama-13B & & & & & & \\
    %ChatLaw-33B & & & & & & \\
    
    \bottomrule[1pt]	
    \end{tabular}
}
% \vspace{-1em}
\caption{The accuracy of evaluated LLMs on H-Law and A-law without human filtering. ``Base'' column indicates the original performance of each LLM. ``Retrieval'' column represented the performance of each LLM argumented by the retrieval. Here we show the results with a maximum retrieval context length of up to 1000 for fair comparisons. ``Oracle'' column stands for the results of using rules, utilized to generate the questions, to argument the LLM.}
\label{tab:law_results}
\end{table*}
